Twisted Hilbert Spaces of 3d Supersymmetric Gauge Theories

We study aspects of 3d $\mathcal{N}=2$ supersymmetric gauge theories on the product of a line and a Riemann surface. Performing a topological twist along the Riemann surface leads to an effective supersymmetric quantum mechanics on the line. We propose a construction of the space of supersymmetric ground states as a graded vector space in terms of a certain cohomology of generalized vortex moduli spaces on the Riemann surface. This exhibits a rich dependence on deformation parameters compatible with the topological twist, including superpotentials, real mass parameters, and background vector bundles associated to flavour symmetries. By matching spaces of supersymmetric ground states, we perform new checks of 3d abelian mirror symmetry.

==> ArXiv Submission 2/preamble.tex <==
%-------------------------------------------------------------


\usepackage{amsfonts}
\usepackage{amscd}
\usepackage{amssymb}
\usepackage{amsmath,bbm}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{tabu}
\usepackage{latexsym}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{tikz-cd}
\usepackage[vcentermath]{youngtab}
%\hypersetup{colorlinks=true, linkcolor=black,citecolor=black,filecolor=black,urlcolor=black,}
    
%-------------------------------------------------------------

\newcommand{\pathtodiagrams}{figures/}

\newcommand{\mathfig}[2]{{\hspace{-3pt}\begin{array}{c}%
  \raisebox{-2.5pt}{\includegraphics[width=#1\textwidth]{\pathtodiagrams #2}}%
\end{array}\hspace{-3pt}}}

\newcommand{\afnote}[1]{\textcolor{blue}{[#1]}}
\newcommand{\mbnote}[1]{\textcolor{red}{[#1]}}


%--------------------------------------------------------------

\def \be  {\begin{equation}}
\def \ee  {\end{equation}}
\def \bea {\begin{equation}\begin{aligned}}
\def \eea {\end{aligned}\end{equation}}
\def \ba  {\begin{eqnarray}}
\def \ea  {\end{eqnarray}}
\def \bb  {\begin{thebibliography}}
\def \eb  {\end{thebibliography}}
\def \lab #1 {\label{#1}}
\def\Re{{\rm Re}} \def\Im{{\rm Im}}

%-------------------------------------------------------------

\newcommand\ep{\epsilon}
\newcommand\bep{\bar\epsilon}

\newcommand\sym{\mathrm{Sym}}
\newcommand\eff{\mathrm{eff}}

\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cJ{\mathcal{J}}
\newcommand\cK{\mathcal{K}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}
\newcommand\cP{\mathcal{P}}
\newcommand\cQ{\mathcal{Q}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cT{\mathcal{T}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}
\newcommand\cW{\mathcal{W}}
\newcommand\cY{\mathcal{Y}}
\newcommand\cZ{\mathcal{Z}}
\newcommand\al{\alpha}
\newcommand\si{\sigma}
\newcommand\dal{\dot\alpha}
\newcommand\Qbar{\bar{Q}}
\newcommand\rf{*}
\newcommand\U{\Upsilon}
\newcommand\q{\mathfrak{q}}
\newcommand\af{\mathfrak{a}}
\newcommand\tf{\mathfrak{t}}
\newcommand\fl{\mathfrak{l}}
\newcommand\qf{\mathfrak{q}}
\newcommand\pf{\mathfrak{p}}
\newcommand\xf{\mathfrak{x}}
\newcommand\slf{\mathfrak{sl}}
\newcommand\C{\mathbb{C}}
\newcommand\Ext{\mathrm{Ext}}

\newcommand\mr{\mathrm{m}}
\newcommand\bC{\mathbb{C }}
\newcommand\bP{\mathbb{P}}
\newcommand\bQ{\mathbb{Q}}
\newcommand\bR{\mathbb{R}}
\newcommand\bT{\mathbb{T}}
\newcommand\bZ{\mathbb{Z}}
\newcommand\R{\mathbb{R}}

\newcommand\SU{\mathrm{SU}}
\newcommand\rD{\mathrm{D}}
\newcommand\rP{\mathrm{P}}
\newcommand\rU{\mathrm{U}}
\newcommand\rW{\mathrm{W}}
\newcommand\rZ{\mathrm{Z}}
\newcommand\ru{\mathrm{u}}

\newcommand\rd{\mathrm{d}}
\newcommand\e{\mathrm{e}}
\newcommand\im{\mathrm{i}}

\newcommand\fm{\mathfrak{m}}
\newcommand\ft{\mathfrak{t}}
\newcommand\fn{\mathfrak{n}}


\newcommand\lb{\lambda}
\newcommand\tlb{\tilde{\lambda}}
\newcommand\teta{\tilde{\eta}}
\newcommand\la{\langle}
\newcommand\ra{\rangle}
\newcommand\del{\partial}
\newcommand\delbar{\bar{\partial}}
\newcommand\Dbar{\bar{\mathcal{D}}}
\newcommand\tr{\mathrm{Tr}}
\newcommand\SUN{\mbox{SU}(N)}
\newcommand\ir{\mathrm{IR}}
\newcommand\uv{\mathrm{UV}}
\newcommand\Hom{\mathrm{Hom}}

\newcommand\rrangle{\ra\ra}
\newcommand{\PE}[1]{ \mathrm{PE}\left[ #1 \right] }
\newcommand{\nn}{\nonumber}

\newcommand\filledcirc{{\color{red}\bullet}\mathllap{\circ}}

%-----------------------------------------------------------------

\definecolor{cardinal}{rgb}{0.6,0,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{golden}{rgb}{0.92, 0.7, 0}
\definecolor{midnight}{rgb}{0, 0, 0.5}
\definecolor{darkblue}{rgb}{0.2, 0, 0.8}
\newcommand{\Red}{\color{red}}
\newcommand{\Blue}{\color{blue}}
\newcommand{\DarkGreen}{\color{darkgreen}}
\newcommand{\Cardinal}{\color{cardinal}}
\newcommand{\Golden}{\color{golden}}
\newcommand{\Midnight}{\color{midnight}}
\newcommand{\DarkBlue}{\color{darkblue}}
\def\DG{\DarkGreen}
\def\CR{\Cardinal}
\def\DB{\DarkBlue}







==> preamble.tex <==
%-------------------------------------------------------------


\usepackage{amsfonts}
\usepackage{amscd}
\usepackage{amssymb}
\usepackage{amsmath,bbm}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{tabu}
\usepackage{latexsym}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{tikz-cd}
\usepackage[vcentermath]{youngtab}
%\hypersetup{colorlinks=true, linkcolor=black,citecolor=black,filecolor=black,urlcolor=black,}
    
%-------------------------------------------------------------

\newcommand{\pathtodiagrams}{figures/}

\newcommand{\mathfig}[2]{{\hspace{-3pt}\begin{array}{c}%
  \raisebox{-2.5pt}{\includegraphics[width=#1\textwidth]{\pathtodiagrams #2}}%
\end{array}\hspace{-3pt}}}

\newcommand{\afnote}[1]{\textcolor{blue}{[#1]}}
\newcommand{\mbnote}[1]{\textcolor{red}{[#1]}}


%--------------------------------------------------------------

\def \be  {\begin{equation}}
\def \ee  {\end{equation}}
\def \bea {\begin{equation}\begin{aligned}}
\def \eea {\end{aligned}\end{equation}}
\def \ba  {\begin{eqnarray}}
\def \ea  {\end{eqnarray}}
\def \bb  {\begin{thebibliography}}
\def \eb  {\end{thebibliography}}
\def \lab #1 {\label{#1}}
\def\Re{{\rm Re}} \def\Im{{\rm Im}}

%-------------------------------------------------------------

\newcommand\ep{\epsilon}
\newcommand\bep{\bar\epsilon}

\newcommand\sym{\mathrm{Sym}}
\newcommand\eff{\mathrm{eff}}

\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cJ{\mathcal{J}}
\newcommand\cK{\mathcal{K}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}
\newcommand\cP{\mathcal{P}}
\newcommand\cQ{\mathcal{Q}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cT{\mathcal{T}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}
\newcommand\cW{\mathcal{W}}
\newcommand\cY{\mathcal{Y}}
\newcommand\cZ{\mathcal{Z}}
\newcommand\al{\alpha}
\newcommand\si{\sigma}
\newcommand\dal{\dot\alpha}
\newcommand\Qbar{\bar{Q}}
\newcommand\rf{*}
\newcommand\U{\Upsilon}
\newcommand\q{\mathfrak{q}}
\newcommand\af{\mathfrak{a}}
\newcommand\tf{\mathfrak{t}}
\newcommand\fl{\mathfrak{l}}
\newcommand\qf{\mathfrak{q}}
\newcommand\pf{\mathfrak{p}}
\newcommand\xf{\mathfrak{x}}
\newcommand\slf{\mathfrak{sl}}
\newcommand\C{\mathbb{C}}
\newcommand\Ext{\mathrm{Ext}}

\newcommand\mr{\mathrm{m}}
\newcommand\bC{\mathbb{C }}
\newcommand\bP{\mathbb{P}}
\newcommand\bQ{\mathbb{Q}}
\newcommand\bR{\mathbb{R}}
\newcommand\bT{\mathbb{T}}
\newcommand\bZ{\mathbb{Z}}
\newcommand\R{\mathbb{R}}

\newcommand\SU{\mathrm{SU}}
\newcommand\rD{\mathrm{D}}
\newcommand\rP{\mathrm{P}}
\newcommand\rU{\mathrm{U}}
\newcommand\rW{\mathrm{W}}
\newcommand\rZ{\mathrm{Z}}
\newcommand\ru{\mathrm{u}}

\newcommand\rd{\mathrm{d}}
\newcommand\e{\mathrm{e}}
\newcommand\im{\mathrm{i}}

\newcommand\fm{\mathfrak{m}}
\newcommand\ft{\mathfrak{t}}
\newcommand\fn{\mathfrak{n}}


\newcommand\lb{\lambda}
\newcommand\tlb{\tilde{\lambda}}
\newcommand\teta{\tilde{\eta}}
\newcommand\la{\langle}
\newcommand\ra{\rangle}
\newcommand\del{\partial}
\newcommand\delbar{\bar{\partial}}
\newcommand\Dbar{\bar{\mathcal{D}}}
\newcommand\tr{\mathrm{Tr}}
\newcommand\SUN{\mbox{SU}(N)}
\newcommand\ir{\mathrm{IR}}
\newcommand\uv{\mathrm{UV}}
\newcommand\Hom{\mathrm{Hom}}

\newcommand\rrangle{\ra\ra}
\newcommand{\PE}[1]{ \mathrm{PE}\left[ #1 \right] }
\newcommand{\nn}{\nonumber}

\newcommand\filledcirc{{\color{red}\bullet}\mathllap{\circ}}

%-----------------------------------------------------------------

\definecolor{cardinal}{rgb}{0.6,0,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{golden}{rgb}{0.92, 0.7, 0}
\definecolor{midnight}{rgb}{0, 0, 0.5}
\definecolor{darkblue}{rgb}{0.2, 0, 0.8}
\newcommand{\Red}{\color{red}}
\newcommand{\Blue}{\color{blue}}
\newcommand{\DarkGreen}{\color{darkgreen}}
\newcommand{\Cardinal}{\color{cardinal}}
\newcommand{\Golden}{\color{golden}}
\newcommand{\Midnight}{\color{midnight}}
\newcommand{\DarkBlue}{\color{darkblue}}
\def\DG{\DarkGreen}
\def\CR{\Cardinal}
\def\DB{\DarkBlue}






